Affect Recognition in Ads with Application to Computational Advertising

Advertisements (ads) often include strongly emotional content to leave a lasting impression on the viewer. This work (i) compiles an affective ad dataset capable of evoking coherent emotions across users, as determined from the affective opinions of five experts and 14 annotators; (ii) explores the efficacy of convolutional neural network (CNN) features for encoding emotions, and observes that CNN features outperform low-level audio-visual emotion descriptors upon extensive experimentation; and (iii) demonstrates how enhanced affect prediction facilitates computational advertising, and leads to better viewing experience while watching an online video stream embedded with ads based on a study involving 17 users. We model ad emotions based on subjective human opinions as well as objective multimodal features, and show how effectively modeling ad emotions can positively impact a real-life application.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

==> user_study.tex <==
Given that superior ad AR is achieved with user EEG responses (see Table \ref{tab:uscap}), we examined if enhanced AR resulted in the insertion of appropriate ads at vantage temporal positions within a streamed video, as discussed in the CAVVA video-in-video ad insertion framework~\cite{cavva}. CAVVA is an optimization-based framework for ad insertion onto streamed videos (as with \textit{YouTube}). It formulates an advertising schedule by modeling the emotional relevance between video scenes and candidate ads to determine (a) the subset of ads for insertion, and (b) the temporal positions (typically after a scene ending) at which the chosen ads are to be inserted. In effect, CAVVA aims to strike a balance between (a) maximizing ad impact in terms of brand memorability, and (b) minimally disrupting (or enhancing) viewer experience while watching the program video onto which ads are inserted. We hypothesized that better ad affect recognition should lead to optimal ad insertions, and consequently better viewing experience. To this end, we performed a user study to compare the subjective quality of advertising schedules generated via ad asl and val scores generated with the content-centric \textbf{Han}~\cite{Hanjalic2005} and \textbf{Deep} CNN models, and the user-centric \textbf{EEG} model. A detailed description of the user study follows. 

\subsection{Dataset}\label{US-DS} 

For performing the user study, we used 28 ads (out of the 100 in the original dataset), and three program videos. The ads were equally divided into four quadrants of the valence-arousal plane based on asl and val labels provided by experts. The program videos were scenes from a television sitcom (\textit{friends}) and two movies (\textit{ipoh} and \textit{coh}), which predominantly comprised social themes and situations capable of invoking high-to-low valence and moderate arousal (see Table~\ref{tab:progdetails} for summary statistics). Each of the program videos comprised eight scenes implying that there were seven candidate ad-insertion points in the middle of each sequence. The average scene length was found to be 118 seconds.

\begin{table}[t]
\fontsize{8}{8}\selectfont
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Summary of program video statistics.}\vspace{-.2cm}
\begin{tabular}{|c|c|cc|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  %\textbf{} & \textbf{Valence}  & \textbf{Arousal} \\   \hline
	\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Scene length (s)}} & \multicolumn{2}{c|}{\textbf{Manual Rating}} \\
	 \hline 
	\multicolumn{1}{|c|}{~} & {~} & {\textbf{Valence}} & {\textbf{Arousal}}\\ \hline
	\textbf{coh}  & 127$\pm$46 & {0.08$\pm$1.18} & {1.53$\pm$0.58}\\
	\textbf{ipoh}  & 110$\pm$44 & {0.03$\pm$1.04} & {1.97$\pm$0.49}\\
	\textbf{friends}  & 119$\pm$69 & {1.08$\pm$0.37} & {2.15$\pm$0.65}\\
\hline
\end{tabular}
\vspace{-.2cm}
\label{tab:progdetails}
\end{table}

\subsection{Advertisement insertion strategy}~\label{US-AdIns}
We used the three aforementioned models to perform ad affect estimation. For the 24 program video scenes (3 videos $\times$ 8 scenes), the average of asl and val ratings acquired from three experts was used to denote affective scores. For the ads, affective scores were computed as follows. For the \textbf{Deep} method, we used normalized softmax class probabilities~\cite{bishop:2013} output by the video-based CNN model for val estimation, and probabilities from the audio CNN for asl estimation. The mean score over all video/audio ad frames was used to denote the affective score in this method. The average of the per-second asl and val level estimates over the ad duration was used to denote affective scores for the \textbf{Han} approach. Mean of SVM class posteriors over all EEG epochs was used for the \textbf{EEG} method. We then adopted the CAVVA optimization framework~\cite{cavva} to obtain nine unique \textbf{video program sequences} (with average length of 19.6 minutes) comprising the inserted ads. These video program sequences comprised ads inserted via the three affect estimation approaches onto each of the three program videos. Exactly five ads were inserted (out of seven possible) onto each program video. 21 of the 28 chosen ads were inserted at least once into the nine video programs, with maximum and mean insertion frequencies of 5 and 2.14 respectively.

\subsection{Experiment and Questionnaire Design}~\label{US-Ques}

To evaluate the subjective quality of the generated video program sequences and thereby the utility of the three affect estimation techniques for computational advertising, we recruited 12 users (5 female, mean age 19.3 years) who were university undergraduates/graduates. Each of these users viewed a total of three {video program sequences}, corresponding to the three program videos with ad insertions performed using \textit{one} of the three affect estimation approaches.  We used a randomized 3$\times$3 Latin square design in order to cover all the nine generated sequences with every set of three users. Thus, each {video program sequence} was seen by four of the 12 viewers.

We designed a questionnaire for the user evaluation so as to reveal whether the generated video program sequences (a) included seamless ad insertions, (b) facilitated user engagement (or alternatively, resulted in minimum disruption) towards the streamed video and inserted ads and (c) ensured good overall viewer experience. To this end, we evaluated whether a particular ad insertion strategy resulted in (i) increased brand recall (both \textit{immediate} and \textit{day-after} recall) and (ii) minimal viewer disturbance or enhanced user viewing experience. 

Recall evaluation to intended to verify if the inserted ads were attended to by viewers, and the immediate and day-after recall were \textit{\textbf{objective}} measures that quantified the impact of ad insertion on the short-term (immediate) and long-term (day-after) memorability of advertised content, upon viewing the program sequences. Specifically, we measured the proportion of (i) inserted ads that were recalled correctly (\textit{Correct} recall), (ii) inserted ads that were not recalled (\textit{Forgotten}) and (iii) non-inserted ads incorrectly recalled as viewed (\textit{Incorrect} recall). For those inserted ads which were correctly recalled, we also assessed whether viewers perceived them to be contextually (emotionally) relevant to the program content.

Upon viewing a video program sequence, the viewer was provided with a representative visual frame from each of the 28 ads  to test ad recall along with a sequence-specific response sheet. In addition to the recall related questions, we asked viewers to indicate if they felt that the recalled ads were inserted at an appropriate position in the video (\textit{Good insertion}) to verify if ad positioning positively influenced recall. All recall and insertion quality-related responses were acquired from viewers as binary values. In addition to these objective measures, we defined a second set of \textit{\textbf{subjective}} user experience measures, and asked users to provide ratings on a Likert scale of 0--4 for the following questions with 4 implying \textit{best} and 0 denoting \textit{worst}:

\begin{itemize}[noitemsep,nolistsep]
\item[1.]Were the advertisements uniformly distributed across the video program?
\item[2.]	Did the inserted advertisements blend with the program flow?
\item[3.]	Whether the inserted ads were relevant to the surrounding scenes with respect to their content and mood?
\item[4.]	What was the overall viewer experience while watching each video program?
\end{itemize}

Each participant filled the recall and experience-related questionnaires immediately after watching each video program\footnote{An exemplar video program sequence is available as supplementary material.}. Viewers also filled in the day-after recall questionnaire, a day after completing the experiment.

\begin{figure*}[t]
\centerline{\includegraphics[width=0.33\linewidth,height=3cm]{Imm_Recall}\hspace{0.05cm}
\includegraphics[width=0.33\linewidth,height=3cm]{DA_Recall}\hspace{0.05cm}
\includegraphics[width=0.33\linewidth,height=3cm]{Sub_exp}}
\centerline{\textbf{Immediate Recall}\hspace{0.2\linewidth}\textbf{Day-after recall}\hspace{0.23\linewidth}\textbf{User Experience}} \vspace{-.2cm}
\caption{\label{US_results} Summary of user study results in terms of recall and user experience-related measures. Error bars denote unit standard deviation.}
\vspace{-.2cm}
\end{figure*}


\subsection{Results and Discussion}

%In this user study, we have used valence and arousal scores derived from (a) EEG recordings (b) deep convolutional models trained on affective datasets and (c) popular computational features ~\cite{Hanjalic2005} and evaluted the performance computational video-in-video advertisement insertion. We have used the framework defined in ~\cite{cavva} which attempts to match valence and arousal ratings for video segments and candidate advertisements. The method in \cite{cavva} simultaneously finds the optimal set of advertisement insertion points, subset of advertisements to be inserted as well as the best assignment of each chosen advertiesment to an insertion point in the video program stream. The performance of this method critically hinges on the  valence and arousal ratings assigned to advertisements as well as video program segments. \\

As mentioned previously, scenes from the program videos were assigned asl, val scores based on manual ratings from three experts, while the Deep, Han and EEG-based methods were employed to compute affective scores for ads. The overall quality of the CAVVA-generated video program sequence hinges on the quality of affective ratings assigned to both the video scenes and ads. In this regard, we hypothesized that better ad affect estimation would result in optimized ad insertions. 

Firstly, we computed the similarity in terms of the ad asl and val scores generated by the three approaches in terms of Pearson correlations, and found that (1) there was significant and positive correlation between asl scores generated by the Han--EEG ($\rho = 0.5, p<0.01$) as well as the Han--Deep methods ($\rho = 0.42, p<0.05$). However, the Deep and EEG-based asl scores did not agree significantly ($\rho = 0.22, \text{n.s.}$). For val, the only significant correlation was noted between the Han and Deep approaches ($\rho = 0.41, p<0.05$), while the Han and EEG ($\rho = 0.07, \text{n.s.}$) as well as the Deep and EEG val scores ($\rho = 0.20, \text{n.s.}$) were largely uncorrelated. This implies that while methods content-centric and user-centric methods agree well on asl scores, there is significant divergence between the val scores generated by the two approaches.

Based on the questionnaire responses received from viewers, we computed the mean proportions for correct recall, ad forgottenness, incorrect recall and good insertions immediately and a day after the experiment. Figure~\ref{US_results} presents the results of our user study and there are several interesting observations. A key measure indicative of a successful advertising strategy is \textit{high brand recall}~\cite{Holbrook1984, cavva, YadatiMMM2013}, and the immediate and day-after recall rates observed for three considered approaches are presented in Fig.~\ref{US_results}(left),(middle). Video program sequences obtained with {Deep} affective scores result in high immediate and day-after recall, least ad forgottenness and least incorrect recall. Ads inserted via the EEG method are found to be the best inserted, even if they have relatively lower recall rates as compared to the Deep approach ($p < 0.05$ for independent $t$-test). Ads inserted via Han-generated affective scores have the least immediate recall and are also forgotten the most, and are also perceived as the the worst inserted. The trends observed for immediate and day-after recall are slightly different, but the various recall measures are clearly worse for the day-after condition with a very high proportion of ads being forgotten. Nevertheless, the observed results clearly suggest that the Deep and EEG approaches which achieve superior AR compared to the Han method also lead to better ad memorability. 

However, it needs to be noted that higher ad recall does not directly translate to a better viewing experience while watching the video programs. On the contrary, some ads may well be remembered because they disrupted the program flow and distracted viewers. In order to examine the impact of the affect-based ad insertion strategy on viewing experience, we computed the mean subjective scores acquired from users (Fig.~\ref{US_results}(right)). Here again, the Deep method scores best in terms of uniform insertion and ad relevance, while the EEG method performs best with respect to blending and viewer experience ($p < 0.05$ with two-sample $t$-tests in all cases). Interestingly, the Han method again performs worst in terms of ad relevance and viewer experience. The CAVVA optimization framework~\cite{cavva} has two components-- one for selection of ad insertion points into the program video, and another for selecting the set of ads to be inserted. Asl scores only play a role in the choice of insertion points, whereas val scores influence both components. In this context, the two best methods for val recognition, which also outperform the Han approach for asl recognition,  maximize both ad recall and viewing experience. 



